Efficient sparsity adaptive changepoint estimation

We propose a new, computationally efficient, sparsity adaptive changepoint estimator for detecting changes in unknown subsets of a high-dimensional data sequence. Assuming the data sequence is Gaussian, we prove that the new method successfully estimates the number and locations of changepoints with a given error rate and under minimal conditions, for all sparsities of the changing subset. Moreover, our method has computational complexity linear up to logarithmic factors in both the length and number of time series, making it applicable to large data sets. Through extensive numerical studies we show that the new methodology is highly competitive in terms of both estimation accuracy and computational cost. The practical usefulness of the method is illustrated by analysing sensor data from a hydro power plant. An efficient R implementation is available.

==> sections/knownsparsity.tex <==
\section{Known sparsity}\label{secknownsparsity}
In this section we present an algorithm for change-point detection and localization for when all changes in mean occur in the same known number of coordinates. Assume that $k_j = k$ for all $j \in [J]$ and some sparsity level $k$. For ease of reading, also assume that $\sigma=1$.

To identify and localize change-points we will aggregate thresholded CUSUM statistics over coordinates. Let $X_{\cdot, i}$ denote the $i$-th row of $X$, containing all observations of the $i$-th coordinate of the responses. Our choice of thresholding value is given by
\begin{equation}
a^2(k) = \begin{cases} 4 \log \left(    \frac{ep \log n^4}{k^2}   \right), & \text{if } k \leq \sqrt{p \log n^4}\\
0, &\text{otherwise. }
\end{cases}
\end{equation}
For any $a>0$ let $\nu_a = \EE \left( Z^2 \ | \ |Z|>a \right)$. For any candidate interval $\{s+1, \ldots, e\}$ and candidate change-point location $b$, with $0\leq s<b< e\leq n$, we take our test statistic to be
$$
T^{b}_{(s,e]}(k) = \sum_{i=1}^p\left( \mathcal{C}^b_{(s,e]}(X_{\cdot, i})^2  - \nu_{a(k)} \right ) \ind_{\left\{\left|\mathcal{C}^b_{(s,e]}(X_{\cdot, i})\right| > a(k) \right\}} ,
$$
where for any $y \in \RR^n$, $\mathcal{C}^b_{(s,e]}(y)$ is the CUSUM computed on $(y_{s+1}, \ldots, y_{e})\T$ evaluated in $b$, that is
\begin{align}
\mathcal{C}^b_{(s,e]}(y):&= \sqrt{\frac{e-b}{(e-s)(b-s)}}\sum_{t=s+1}^b y_t - \sqrt{\frac{b-s}{(e-s)(e-b)}}\sum_{t=b+1}^e y_t.
\end{align}
\newline\newline
Now that we have a statistic for testing whether or not the interval $(s,e]$ contains a change-point at $b$, we can use it to construct a multiple change-point procedure. The idea is to take the test statistic for a single change and combine it with a search procedure for multiple changes. Our choice of such a search procedure is Seeded Binary Segmentation (SBS). SBS is a variant of Wild Binary Segmentation (WBS) with non-randomly generated candidate intervals. The idea of WBS is that certain arrangements of change-points within a segment may obfuscate the CUSUM statistic over the segment and weaken the ability of the CUSUM statistic to detect a change-point. The solution, then, is to look for changes in candidate segments of varying lengths and placements. \n\n
% \textbf{Algorithm.}\newline
We now describe the HDCD algorithm. We begin by describing the generation of \textit{seeded intervals}. We introduce a slight variant to the Seeded Intervals presented in \citet{kovacs_seeded_2020}. Let $\alpha>1$ and $D\in \NN$ be tuning parameters. We will iterate through a sequence of interval lengths, where we increase the length by multiplying the previous length by $\alpha$, and for a fixed interval length $l$, we will generate intervals by shifting the previous interval to the right by at most $\frac{l}{D}$.\newline\newline
\textit{Note: For two integers $s<e$, we write $(s,e]$ to mean the integer interval $\{s+1, \ldots, e\}$. Moreover, by the "length" of $(s,e]$, we mean $e-s$.}
\begin{algorithm}[H]
\caption{Seeded Interval Generation$(\alpha, D)$}\label{alg:seededintervals}
\begin{algorithmic}
\Require $\alpha>1, D\geq 1$
\State $\text{Intervals} \gets \{\}$
\State $l \gets 2$ \Comment{$l$ is current interval length}
\While{$l \leq n$}
    \State $s = \max \left\{ 1, \lfloor \frac{l}{D} \rfloor\right\}$ \Comment{$s$ is current interval shift}
    \For{$i = 0, \ldots, \left\lfloor \frac{n-l}{s} \right \rfloor$}
        \State $\text{Intervals} \gets \text{Intervals}\cup \{(is, is+l]\}$
    \EndFor
    \State $l\gets \max \left\{l+1, \left \lfloor \alpha l \right \rfloor\right\}$
\EndWhile
\State \Return Intervals.
\end{algorithmic}
\end{algorithm}
Define the recursive sequence $(l_j)_{j \in \NN}$ by $l_1 = 2$, and $l_{j+1} = \max \left\{l+1,  \lfloor \alpha l_j\rfloor \right\}$ for $j\in \NN$. Let $J = \sup \{ j \in \NN \ : \ l_j \leq n\}$. Formally, the set $\mathcal{S}$ of seeded intervals is given by
\begin{align}
\mathcal{S} &= \bigcup_{l \in \{l_1, \ldots, l_J\}}  \mathcal{I}_l,
\intertext{where}
\mathcal{I}_l &= \bigcup_{i=0}^{\lfloor \frac{n-l}{s_l}\rfloor} \left\{(i s_l \ , \ i s_l +l ]\right\}\\
s_l &= \max \left\{ 1, \left\lfloor \frac{l}{D} \right\rfloor\right\}.
\end{align}
\n\n
The point is that each relative increase in length of the intervals is bounded above by $\alpha$, and that for a given interval length $l$, each consecutive interval is shifted by at most $\frac{l}{D}$. \n\n

% Informally, we first generate intervals of length $1$:
% \begin{align}
% (s_1, e_1] &= (0,2] = [1,2]\\
% (s_2, e_2] &= (1,3] = [2,3]\\
% &\vdots\\
% (s_{n-1}, e_{n-1}] &= (n-2, n] = [n-1,n].
% \end{align}
% Then generate intervals of lengths $l = 2, 3,\dots, \lceil \frac{1}{\alpha-1} \rceil+1$, where each consecutive interval is shifted to the right by $ \max \left\{ 1, \lfloor \frac{l}{D} \rfloor\right\}$. For all $l \geq \lceil \frac{1}{\alpha-1} \rceil$, we have that $\alpha l \geq l-1$ [ DOUBLE CHECK!!!!!].
% So continue generating intervals in the following recursive fashion. Set $l = \left \lfloor \frac{\alpha}{\alpha-1} \right \rfloor$. While $l \leq n$, proceed by
% \begin{itemize}
%     \item Define the shift by $s = \max \left\{ 1, \lfloor \frac{l}{D} \rfloor\right\}$.
%     \item Generate intervals $(0, l]$, $(s, l + s], \cdots, (\tau s, l + \tau s]$, where
%     $\tau$ is the largest integer such that $l + \tau s \leq n$. 
%     \item Set $l \leftarrow \left \lfloor \alpha l \right \rfloor$.
% \end{itemize}
% Let $M$ be the total number of intervals.\newline\newline
% Formally, the set of seeded intervals are given by
% $$\mathcal{S} \cup \mathcal{L},$$
% where
% \begin{align}
% \mathcal{S} &= \bigcup_{l=1}^{\left \lceil\frac{1}{\alpha-1} \right\rceil+1} \mathcal{I}_l,\\
% \mathcal{I}_l &= \bigcup_{v=1}^{\lfloor \frac{n-l}{s_j}\rfloor} \left\{(v s_l, l + vs_l ]\right\}\\
% s_l &= \max \left\{ 1, \left\lfloor \frac{l}{D} \right\rfloor\right\}
% \intertext{and, letting $l^{(j)}$ for $j\geq 1$ be the recursive sequence defined by $l^{(1)} = \left \lfloor \frac{\alpha}{\alpha-1} \right \rfloor$, and $l^{(j+1)} = \lfloor \alpha l^{(j)}\rfloor$, and $J = \max \{ j  \ : \ l^{(j)} \leq n\}$}
% \mathcal{L}&= \bigcup_{l \in \{l^{(1)}, l^{(2)}, \ldots, \l^{(J)}\}} \mathcal{I}_{l}.
% \end{align}
% \n\n
% The point is that each relative increase in length of the intervals is bounded above by $\alpha$, and that for a given interval length $l$, each consecutive interval is shifted by at most $\frac{l}{D}$. \n\n

The High Dimensional Change-point Detection algorithm is defined in the following recursive way. 
Given observations $X \in \RR^{p \times n}$, a sparsity level $k$, threshold $\xi>0$, and $M$ seeded intervals $\mathcal{S} = \{(s_m, e_m] \ ; \ m\in [M]\}$ generated from algorithm \ref{alg:seededintervals} the HDCD algorithm is initiated by calling HDCD$(X, \xi, (0,n], \mathcal{S} ,\{\})$.\newline
\begin{algorithm}[H]
\caption{HDCD$\left( X, \xi(k), (s, e], \mathcal{S}, \mathcal{B}\right)$}\label{alg:cap}
\begin{algorithmic}
\State \textbf{Input: } Matrix of observations $X \in \RR^{p \times n}$, thresholding constant $\xi(k)$, left open and right closed integer interval $(s,e]$ in which candidate change-points are searched for, an enumerated collection $\mathcal{S} =  \{(s_m, e_m] \ ; \ m\in [M]\}$ of $M$ seeded intervals, a set of already detected change-points $\mathcal{B}$. 
\State \textbf{Output: } Set $\mathcal{B}$ of detected change-points.\n 
\If{$e-s\leq 1$}
    \State STOP.
\EndIf
\State $\mathcal{M}_{(s,e]} = \left\{   m \ : \ (s_m, e_m] \subset (s,e]   \right\}$
\State $\mathcal{O}_{(s,e]} = \left\{   m \in \mathcal{M}_{(s,e]} \ : \ \underset{s_m < b <e_m}{\max} T^{b}_{(s_m,e_m]}(k) > \xi(k)  \right\}$
\If{$\mathcal{O}_{(s,e]} = \emptyset$}
    \State STOP.
\EndIf
\State $l^*= \underset{m \in \mathcal{O}_{(s,e]}}{\text{min}} |e_m - s_m|$
\State $\mathcal{O}_{l^*} = \mathcal{O}_{(s,e]} \bigcap \left\{   m \ : \  |e_m - s_m| = l^* \right\}$
\State $m^*= \underset{m \in \mathcal{O}_{l^*}}{\text{argmax}} \underset{s_m < b <e_m}{\max} T^{b}_{(s_m,e_m]}(k)$
\State $b^*= \underset{s_{m^*} <b <e_{m^*}}{\text{argmax}} T^{b}_{(s_{m^*},e_{m^*}]}(k)$
\State $\mathcal{B} \gets \mathcal{B} \cup \{b^*\}$
\State $\mathcal{B}  \gets \text{HDCD} \left( (s, b^*], \xi(k), \mathcal{S}, \mathcal{B}\right)$
\State $\mathcal{B} \gets \text{HDCD} \left( (b^*,e], \xi(k),\mathcal{S}, \mathcal{B}\right)$
\State \textbf{return} $\mathcal{B}$
\end{algorithmic}
\end{algorithm}
\leavevmode\newline\newline
\TODO{Make more clear that intervals are already generated. Also comment on computational issues like discussed in meeting. Not clear from algorithm that we can stop once we find a wide enough interval.}\n\n
\TODO{Put computational complexity here?}\n\n
By a rough bound be obtain the following. \textbf{Note:} Probably $\mathcal{O}(np \log(np))$ for dense and sparse changes, only dense for now. \n\n
We remark that the above algorithm allows for a great computational speedups thanks to declaring a change-point in the narrowest interval at which the test statistic exceeds the given threshold. To search for a change-point in a given interval $(s,e] \subseteq (0, n]$, one can search for change-points in intervals in order ascending in length.
\begin{proposition}\label{compprop}
For any input matrix $X \in \RR^{p \times n}$, threshold level and seeded intervals generated by Algorithm \ref{alg:seededintervals} with $\alpha>1$ and $D \in \NN$, the computational complexity of HDCD in terms of FLOPS is $\mathcal{O}(np)$ in the best case and $\mathcal{O}(np \log n)$ in the worst case. 
\end{proposition}
\TODO{Double check proof.}
\n\n
We introduce the following notation. For $j=1, \ldots, J$, let $\Delta_j = \min \{\eta_{j+1}- \eta_j, \eta_j - \eta_{j-1}\}$ be the minimum distance between the $j$-th change-point and its two neighbouring change-points (letting $\eta_0 =0$ and $\eta_{J+1} = n$), and $\Delta = \underset{j \in [J]}{\min} \Delta_j$. Let $\phi_j = \normm{\mu_{\eta_{j+1}} - \mu_{\eta_j}}_2$ be the $\ell_2$ norm of the mean-change occuring at change-point $j$. Let $k_j = \min \normm{\mu_{\eta_{j+1}} - \mu_{\eta_j}}_0$ be the number of components undergoing a change at the $j$-th change-point. We have the following consistency result.
% \begin{theorem}\label{densetheorem}
% Suppose that $k_j \geq \sqrt{4 p\log(n)}$ for all $j \in [K]$, so that we are in a \textit{dense} regime. There exist universal constants $C_0, C_1,C_3>0$ such that the following holds. 

% Let $\widehat{K}$ and $\widehat{\eta}_1, \ldots, \widehat{\eta}_{\widehat{K}}$ respectively be estimated number and positions of the change-points from the HDCD procedure, sorted in increasing order, using tuning parameters $\alpha \leq 1 + \frac{1}{6}$, $D\geq 7$, and $\xi^2 = C_1 \sigma^2\sqrt{p \log n}$. If the signal-to-noise condition 
% $$
% \frac{\frac{\phi^2}{\sqrt{p}} \Delta_j}{\sigma^2} \geq C_0 \sqrt{\log n}
% $$holds for all $j \in [K]$, then for all $n\geq 3$ we have that
% \begin{align}
% \mathbb{P} \left(      \widehat{K} = K \ \cap  \underset{j \in [K]}{\max} |\widehat{\eta}_j - \eta_j| \leq C_3 \frac{\sigma^2}{\phi_j^2/\sqrt{p}} \sqrt{\log n}      \right) > 1-\frac{3}{n}.
% \end{align}
% \end{theorem}
\begin{theorem}\label{densetheorem}
Suppose all changes in mean occur in the same (known) number of coordinates, $k_1= \ldots= k_J$. 
Define
\begin{align}
r(k) = \begin{cases}
k \log \left( \frac{e p \log(n^4)}{k^2}\right) \vee \log(n^4), & \text{ if } k \leq \sqrt{p\log(n^4)}\\
\sqrt{p \log(n^4)},& \text{ otherwise}.
\end{cases}
\end{align}
There exist universal constants $C_0, C_1,C_3>0$ such that the following holds. 

Let $\widehat{J}$ and $\widehat{\eta}_1, \ldots, \widehat{\eta}_{\widehat{J}}$ respectively be estimated number and positions of the change-points from the HDCD procedure, sorted in increasing order, with seeded intervals generated from Algorithm \ref{alg:seededintervals} with parameters $\alpha \leq 1 + \frac{1}{6}$, $D\geq 7$, and $\xi(k) = C_1 r(k)$, and input matrix $\widetilde{X} = \left(X_{i,j}/\sigma\right)_{i = 1, \ldots, p; j = 1, \ldots, n}$. If the signal-to-noise condition 
$$
\frac{\phi_j^2}{ \Delta_j}{\sigma^2} \geq C_0 \xi(k)
$$holds for all $j \in [J]$, then for all $n\geq 3$ we have that
\begin{align}
\mathbb{P} \left(      \widehat{J} = J \ \cap  \underset{j \in [J]}{\max} |\widehat{\eta}_j - \eta_j| \leq C_3 \frac{\sigma^2}{\phi_j^2} \xi(k)      \right) > 1-\frac{3}{n}.
\end{align}
\end{theorem}
\n\n
\begin{remark}
The required signal strength is up to a constant factor equal to the information theoretic lower bound on detectable change-points. Ref Pilliat. 
\end{remark}
\begin{remark}
The minimax error rate for estimating change-point $j$ is up to constants given by $\frac{\sigma^2}{\phi_j^2}$. Thus, the estimation error of HDCD is shown to be optimal up to a factor of $\xi(k)$. 
\end{remark}
\begin{remark}
In particular, the above algorithm implies that a Seeded Binary Segmentation scheme based on summed squared CUSUMs is consistent as long as $\frac{\phi_j^2}{ \Delta_j}{\sigma^2} \gg \sqrt{p \log n}$.
\end{remark}
% \begin{remark}
% The constants are quite conservative. We can take $C_0 = 2158$, $C_1 = 200$ and $C_3 = 72$. 
% \end{remark}
% \begin{remark}
% In fact, there exists universal constants $\widetilde{C}_0, \widetilde{C}_1, \widetilde{C}_2,\widetilde{C}_3$ such that the same result holds whenever $\widetilde{C}_1 \sigma^2 \sqrt{p \log n} \leq \xi^2 \leq \widetilde{C}_2 \Delta_j \phi_j^2$ (with $\widetilde{C}_0, \widetilde{C}_3$ replacing $C_0, C_1$).
% \end{remark}
% \begin{remark}
% Suppose that $\frac{\frac{\phi^2}{\sqrt{p}} \Delta_j}{\sigma^2} \gg$\footnote{By $a_n \gg b_n$ we mean that $\frac{b_n}{a_n}\rightarrow 0$}$\log n$. Between two vectors $x \in \RR^{d_1}$, $y \in \RR^{d_2}$, let $H(x,y)$ denote the bi-directional Hausdorff distance [define it]. Let $\eta = (\eta_1, \ldots, \eta_K)\T$ and $\widehat{\eta}=(\widehat{\eta}_1, \ldots, \widehat{\eta}_{\widehat{K}})\T$ be the vectors of true change-points and estimated change-points from the HDCD procedure, respectively, when we choose $\xi^2 = C_1 \sqrt{p\log n}$ for $C_1$ sufficiently large. Then the Theorem implies that
% $$
% H(\widehat{\eta}, \eta) \overset{\text{p}}{\rightarrow}0,
% $$
% as $n \rightarrow \infty$.
% \n\TODO{Check this, not entirely convinced actually...}
% \end{remark}

% \textbf{Conjecture.} (Only based on a hunch)\newline
% Let $k$ be the number of coordinate that undergo a change. If $k \gtrsim \sqrt{2p \log n}$ (a \textit{dense} regime), then if 
% $\frac{\frac{\phi^2}{\sqrt{p}} \Delta}{\sigma^2} \lesssim \sqrt{\log n}$, consistent change-point localization is impossible. However, if $\frac{\frac{\phi^2}{\sqrt{p}} \Delta}{\sigma^2} \gtrsim \sqrt{\log n}$, the minimax estimation error of a change-point is $\asymp \frac{\sigma^2}{\phi^2/\sqrt{p}}$.\newline\newline
% \textit{Reason.}\newline
% If $\frac{\frac{\phi^2}{\sqrt{p}} \Delta}{\sigma^2} \lesssim \sqrt{\log n}$, the signal is not larger than tail-bounds on the Chi square distribution (which I believe are tight or close to tight). \n\n


==> tables/tablemulti/table_copy.tex <==
%%REMEMBER to use package \usepackage{rotating}!!
 \begin{table}[H] \centering
\caption{Multiple change-point estimation}
\label{fig:tablemulti}
\small
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{\extracolsep{1pt}} cccc|cccccc|cccccc|cccccc}
\hline
\multicolumn{4}{c|}{Parameters} & \multicolumn{6}{c|}{Hausdorff distance} &\multicolumn{6}{c|}{$\left | \widehat{K}-K \right |$}  &\multicolumn{6}{c}{Time in miliseconds} \\ \hline 
$n$ & $p$ & Sparsity & K & \text{FAST}  & \text{Pilliat} & \text{Inspect} & \text{SBS} & \text{SUBSET}  & \text{DC} & \text{FAST}  & \text{Pilliat} & \text{Inspect} & \text{SBS} & \text{SUBSET}  & \text{DC} &\text{FAST} & \text{Pilliat} & \text{Inspect} & \text{SBS} & \text{SUBSET}  & \text{DC}  \\
\hline \
200 & 100 & - & 0  & -  & -  & -  & -  & -  & -  & \textbf{0.000}  & \textbf{0.000}  & \textbf{0.000}  & 0.035 & 0.001 & 0.043 & \textbf{14.062}  & 32.102 & 78.490 & 233.022 & 237.610 & 284.542 \\
200 & 100 & Dense & 2  & \textbf{5.273}  & 23.045 & 21.610 & 69.918 & 6.516 & 76.367 & \textbf{0.059}  & 0.477 & 0.286 & 1.028 & 0.108 & 1.076 & \textbf{13.548}  & 28.314 & 65.429 & 232.714 & 416.144 & 296.487 \\
200 & 100 & Sparse & 2  & \textbf{1.427}  & 12.539 & 7.920 & 49.193 & 1.667 & 14.918 & \textbf{0.009}  & 0.245 & 0.103 & 0.695 & 0.035 & 0.260 & \textbf{13.258}  & 27.534 & 60.603 & 234.747 & 421.068 & 303.679 \\
200 & 100 & Mixed & 2  & 4.598 & 18.566 & 14.355 & 61.153 & \textbf{3.741}  & 52.926 & \textbf{0.051}  & 0.356 & 0.188 & 0.867 & 0.062 & 0.742 & \textbf{13.359}  & 27.815 & 62.564 & 235.707 & 419.699 & 300.312 \\
200 & 100 & Dense & 5  & \textbf{5.172}  & 23.738 & 16.271 & 67.285 & 6.424 & 55.707 & \textbf{0.137}  & 1.530 & 0.540 & 3.198 & 0.330 & 2.759 & \textbf{11.811}  & 23.525 & 45.899 & 234.982 & 455.841 & 305.462 \\
200 & 100 & Sparse & 5  & \textbf{1.359}  & 13.986 & 6.378 & 57.178 & 2.424 & 23.193 & \textbf{0.023}  & 0.799 & 0.228 & 2.786 & 0.204 & 1.361 & \textbf{11.381}  & 22.460 & 40.914 & 235.860 & 456.405 & 305.050 \\
200 & 100 & Mixed & 5  & \textbf{4.042}  & 18.768 & 12.559 & 60.433 & 4.901 & 41.305 & \textbf{0.098}  & 1.197 & 0.421 & 3.008 & 0.281 & 2.164 & \textbf{11.526}  & 22.899 & 43.101 & 235.519 & 448.530 & 305.844 \\
200 & 1000 & - & 0  & -  & -  & -  & -  & -  & -  & \textbf{0.000}  & \textbf{0.000}  & \textbf{0.000}  & 0.340 & 0.024 & 0.017 & \textbf{139.691}  & 436.903 & 701.456 & 1536.568 & 1848.143 & 1732.493 \\
200 & 1000 & Dense & 2  & 1.452 & 13.393 & 9.490 & 55.116 & \textbf{1.079}  & 84.983 & \textbf{0.008}  & 0.279 & 0.119 & 0.721 & 0.031 & 1.232 & \textbf{126.219}  & 365.936 & 527.344 & 1552.658 & 3335.223 & 1801.727 \\
200 & 1000 & Sparse & 2  & 0.830 & 9.074 & 9.830 & 49.716 & \textbf{0.751}  & 20.376 & \textbf{0.003}  & 0.182 & 0.151 & 0.621 & 0.029 & 0.291 & \textbf{123.181}  & 359.008 & 495.239 & 1556.123 & 3330.077 & 1870.396 \\
200 & 1000 & Mixed & 2  & 1.776 & 11.782 & 9.585 & 50.506 & \textbf{1.480}  & 53.226 & \textbf{0.013}  & 0.243 & 0.125 & 0.690 & 0.041 & 0.817 & \textbf{123.299}  & 362.036 & 509.172 & 1551.170 & 3303.686 & 1841.540 \\
200 & 1000 & Dense & 5  & \textbf{1.524}  & 15.808 & 9.328 & 57.330 & 1.558 & 60.791 & \textbf{0.025}  & 1.018 & 0.261 & 2.960 & 0.173 & 3.057 & \textbf{106.818}  & 298.488 & 359.276 & 1565.517 & 3581.977 & 1878.816 \\
200 & 1000 & Sparse & 5  & \textbf{0.685}  & 11.342 & 9.161 & 54.198 & 1.520 & 25.800 & \textbf{0.002}  & 0.639 & 0.357 & 2.684 & 0.167 & 1.428 & \textbf{103.679}  & 290.448 & 330.606 & 1565.495 & 3583.778 & 1903.995 \\
200 & 1000 & Mixed & 5  & \textbf{1.189}  & 13.932 & 9.446 & 58.255 & 1.720 & 45.158 & \textbf{0.017}  & 0.813 & 0.332 & 2.864 & 0.191 & 2.377 & \textbf{105.037}  & 296.019 & 350.919 & 1558.004 & 3592.861 & 1890.228 \\
200 & 5000 & - & 0  & -  & -  & -  & -  & -  & -  & \textbf{0.000}  & \textbf{0.000}  & 0.002 & 1.957 & \textbf{0.000}  & \textbf{0.000}  & \textbf{757.654}  & 2614.839 & 3598.080 & 7364.337 & 8767.308 & 51579.636 \\
200 & 5000 & Dense & 2  & 0.965 & 12.988 & 13.254 & 54.753 & \textbf{0.600}  & 124.337 & \textbf{0.003}  & 0.294 & 0.170 & 0.534 & 0.019 & 1.679 & \textbf{662.223}  & 2169.932 & 2706.666 & 7368.847 & 15686.434 & 49298.941 \\
200 & 5000 & Sparse & 2  & 0.763 & 9.655 & 15.806 & 58.961 & \textbf{0.512}  & 70.825 & \textbf{0.001}  & 0.203 & 0.235 & 0.562 & 0.028 & 1.039 & \textbf{653.419}  & 2149.244 & 2614.277 & 7386.109 & 15778.982 & 48025.551 \\
200 & 5000 & Mixed & 2  & 0.977 & 11.364 & 13.762 & 55.915 & \textbf{0.782}  & 96.945 & \textbf{0.003}  & 0.254 & 0.212 & 0.500 & 0.027 & 1.361 & \textbf{662.092}  & 2163.051 & 2659.395 & 7376.635 & 15707.923 & 49492.414 \\
200 & 5000 & Dense & 5  & \textbf{0.891}  & 14.586 & 12.967 & 50.328 & 1.373 & 83.639 & \textbf{0.009}  & 0.942 & 0.449 & 2.448 & 0.173 & 3.635 & \textbf{555.156}  & 1776.451 & 1865.861 & 7387.111 & 16908.091 & 47356.346 \\
200 & 5000 & Sparse & 5  & \textbf{0.534}  & 11.697 & 13.501 & 53.998 & 1.291 & 54.328 & \textbf{0.000}  & 0.735 & 0.548 & 2.529 & 0.176 & 2.712 & \textbf{541.355}  & 1741.575 & 1733.878 & 7381.276 & 17003.759 & 46295.824 \\
200 & 5000 & Mixed & 5  & \textbf{0.776}  & 13.568 & 13.252 & 53.718 & 1.413 & 69.941 & \textbf{0.004}  & 0.855 & 0.501 & 2.503 & 0.174 & 3.191 & \textbf{554.441}  & 1769.514 & 1813.479 & 7365.522 & 17058.979 & 45805.130 \\
500 & 100 & - & 0  & -  & -  & -  & -  & -  & -  & \textbf{0.000}  & \textbf{0.000}  & \textbf{0.000}  & 0.057 & 0.004 & 0.046 & \textbf{42.531}  & 99.644 & 325.703 & 269.828 & 405.589 & 387.122 \\
500 & 100 & Dense & 2  & 15.310 & 71.171 & 50.125 & 130.610 & \textbf{7.423}  & 140.433 & 0.078 & 0.612 & 0.299 & 0.784 & \textbf{0.048}  & 0.838 & \textbf{41.175}  & 90.886 & 286.769 & 273.386 & 725.083 & 412.094 \\
500 & 100 & Sparse & 2  & \textbf{2.739}  & 30.053 & 15.911 & 66.668 & 3.201 & 21.826 & \textbf{0.003}  & 0.284 & 0.096 & 0.363 & 0.035 & 0.161 & \textbf{40.122}  & 87.715 & 269.637 & 276.899 & 740.639 & 428.325 \\
500 & 100 & Mixed & 2  & 11.309 & 54.753 & 35.821 & 93.890 & \textbf{5.418}  & 88.264 & 0.063 & 0.464 & 0.208 & 0.533 & \textbf{0.038}  & 0.530 & \textbf{40.406}  & 89.075 & 277.789 & 275.989 & 727.036 & 421.694 \\
500 & 100 & Dense & 5  & 20.245 & 66.890 & 50.548 & 120.816 & \textbf{8.226}  & 102.263 & 0.229 & 1.939 & 0.726 & 2.543 & \textbf{0.207}  & 1.988 & \textbf{37.355}  & 79.717 & 221.638 & 277.736 & 768.876 & 441.706 \\
500 & 100 & Sparse & 5  & \textbf{3.591}  & 36.375 & 20.258 & 70.980 & 4.767 & 19.457 & \textbf{0.021}  & 0.923 & 0.301 & 1.605 & 0.191 & 0.513 & \textbf{36.058}  & 75.978 & 201.388 & 281.926 & 783.147 & 455.224 \\
500 & 100 & Mixed & 5  & 12.290 & 53.954 & 39.507 & 104.507 & \textbf{6.803}  & 77.078 & \textbf{0.150}  & 1.489 & 0.582 & 2.138 & 0.193 & 1.441 & \textbf{36.670}  & 78.143 & 213.315 & 280.019 & 789.514 & 446.302 \\
500 & 1000 & - & 0  & -  & -  & -  & -  & -  & -  & \textbf{0.000}  & 0.002 & \textbf{0.000}  & 0.471 & \textbf{0.000}  & 0.025 & \textbf{433.387}  & 1352.754 & 4003.779 & 1867.974 & 3183.342 & 2694.059 \\
500 & 1000 & Dense & 2  & \textbf{2.217}  & 30.635 & 18.859 & 102.138 & 2.790 & 99.626 & \textbf{0.002}  & 0.295 & 0.094 & 0.531 & 0.044 & 0.591 & \textbf{395.318}  & 1180.686 & 2925.165 & 1909.202 & 5705.653 & 2976.791 \\
500 & 1000 & Sparse & 2  & 2.052 & 17.323 & 23.773 & 71.741 & \textbf{1.325}  & 18.185 & \textbf{0.002}  & 0.148 & 0.135 & 0.382 & 0.023 & 0.116 & \textbf{387.795}  & 1159.360 & 2705.861 & 1906.765 & 5685.049 & 3056.583 \\
500 & 1000 & Mixed & 2  & 2.181 & 25.431 & 21.361 & 92.648 & \textbf{1.907}  & 68.446 & \textbf{0.002}  & 0.223 & 0.114 & 0.496 & 0.061 & 0.426 & \textbf{392.737}  & 1174.216 & 2852.914 & 1898.906 & 5738.697 & 3004.698 \\
500 & 1000 & Dense & 5  & \textbf{2.893}  & 36.449 & 25.510 & 97.098 & 3.660 & 86.127 & \textbf{0.015}  & 0.964 & 0.282 & 2.143 & 0.174 & 1.717 & \textbf{350.425}  & 1019.516 & 1939.081 & 1938.180 & 6078.462 & 3215.023 \\
500 & 1000 & Sparse & 5  & \textbf{1.808}  & 22.483 & 22.461 & 66.221 & 4.089 & 20.893 & \textbf{0.001}  & 0.547 & 0.363 & 1.493 & 0.191 & 0.498 & \textbf{341.533}  & 993.649 & 1772.807 & 1947.683 & 6064.842 & 3277.823 \\
500 & 1000 & Mixed & 5  & \textbf{2.526}  & 31.025 & 24.077 & 90.958 & 4.682 & 60.749 & \textbf{0.011}  & 0.768 & 0.315 & 1.847 & 0.213 & 1.216 & \textbf{349.400}  & 1010.753 & 1877.088 & 1935.681 & 6121.370 & 3260.986 \\
500 & 5000 & - & 0  & -  & -  & -  & -  & -  & -  & \textbf{0.000}  & 0.002 & 0.006 & 2.508 & 0.025 & \textbf{0.000}  & \textbf{2428.141}  & 8133.956 & 22494.127 & 9201.129 & 15565.885 & 91558.067 \\
500 & 5000 & Dense & 2  & 2.011 & 34.047 & 21.082 & 139.285 & \textbf{1.647}  & 282.956 & \textbf{0.002}  & 0.329 & 0.105 & 1.106 & 0.030 & 1.562 & \textbf{2214.321}  & 7146.322 & 15783.063 & 9254.045 & 27379.887 & 80696.792 \\
500 & 5000 & Sparse & 2  & 2.033 & 16.974 & 32.140 & 144.237 & \textbf{1.408}  & 132.128 & \textbf{0.002}  & 0.148 & 0.188 & 1.159 & 0.083 & 0.778 & \textbf{2175.921}  & 7005.432 & 15049.144 & 9273.951 & 27180.169 & 78843.414 \\
500 & 5000 & Mixed & 2  & 2.277 & 26.553 & 24.275 & 141.006 & \textbf{1.990}  & 207.933 & \textbf{0.003}  & 0.241 & 0.133 & 1.146 & 0.027 & 1.184 & \textbf{2195.945}  & 7084.571 & 15643.843 & 9288.739 & 27274.167 & 84199.591 \\
500 & 5000 & Dense & 5  & \textbf{1.937}  & 42.354 & 24.293 & 84.334 & 3.570 & 187.785 & \textbf{0.006}  & 1.182 & 0.292 & 1.133 & 0.186 & 3.405 & \textbf{1944.761}  & 6192.690 & 10207.377 & 9349.306 & 28981.513 & 80736.801 \\
500 & 5000 & Sparse & 5  & \textbf{1.671}  & 21.168 & 29.794 & 79.665 & 2.654 & 104.455 & \textbf{0.002}  & 0.560 & 0.500 & 1.073 & 0.150 & 2.029 & \textbf{1878.150}  & 5973.240 & 9474.502 & 9351.447 & 29040.033 & 76410.134 \\
500 & 5000 & Mixed & 5  & \textbf{1.957}  & 31.474 & 25.265 & 84.857 & 3.864 & 143.185 & \textbf{0.006}  & 0.860 & 0.380 & 1.154 & 0.190 & 2.772 & \textbf{1873.035}  & 6047.817 & 9647.494 & 9246.865 & 28358.843 & 78434.671 \\
\hline \multicolumn{4}{c|}{Average}
 & 3.480  & 25.248 & 20.098 & 77.767 & \textbf{3.033} & 81.015 & \textbf{0.025} & 0.549 & 0.246 & 1.385 & 0.104 & 1.263 \\
\hline \\[-1.8ex]
\\[-1.8ex]
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/tablemulti_misspec/table.tex <==
%%REMEMBER to use package \usepackage{rotating}!!
 \begin{table}[h] \centering
\caption{Multiple changepoints under misspecified models}
\label{tablemulti_misspec}
\small
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{\extracolsep{1pt}} cc|cccccc|cccccc}
\hline
\multicolumn{2}{c|}{Parameters} & \multicolumn{6}{c|}{Hausdorff distance} &\multicolumn{6}{c|}{$\left | \widehat{K}-K \right |$}   \\ \hline 
Model  & K & \text{ESAC}  & \text{Pilliat} & \text{Inspect} & \text{SBS} & \text{SUBSET}  & \text{DC} & \text{ESAC}  & \text{Pilliat} & \text{Inspect} & \text{SBS} & \text{SUBSET}  & \text{DC} \\
\hline \
$M$ & 0  & -  & -  & -  & -  & -  & -  & \textbf{0.000}  & \textbf{0.000}  & \textbf{0.000}  & \textbf{0.000}  & \textbf{0.000}  & \textbf{0.000}  \\
$M$ & 3  & 0.917 & 4.583 & 1.083 & 6.000 & \textbf{0.500}  & 32.750 & \textbf{0.000}  & \textbf{0.000}  & \textbf{0.000}  & 0.083 & \textbf{0.000}  & 0.833 \\
$M_{\text{Unif}}$ & 0  & -  & -  & -  & -  & -  & -  & \textbf{0.000}  & \textbf{0.000}  & \textbf{0.000}  & 0.083 & \textbf{0.000}  & \textbf{0.000}  \\
$M_{\text{Unif}}$ & 3  & 0.500 & 33.750 & 5.000 & 7.167 & \textbf{0.417}  & 15.667 & \textbf{0.000}  & 0.833 & 0.083 & 0.083 & \textbf{0.000}  & 0.417 \\
$M_{t_{3}}$ & 0  & -  & -  & -  & -  & -  & -  & 138.750 & 141.667 & 140.167 & \textbf{0.000}  & 101.667 & \textbf{0.000}  \\
$M_{t_{3}}$ & 3  & 48.583 & 48.833 & 48.750 & \textbf{22.917}  & 46.083 & 126.667 & 134.083 & 136.167 & 135.500 & \textbf{0.417}  & 69.417 & 2.750 \\
$M_{t_{10}}$ & 0  & -  & -  & -  & -  & -  & -  & 3.917 & 4.083 & 1.167 & \textbf{0.000}  & 37.500 & \textbf{0.000}  \\
$M_{t_{10}}$ & 3  & 30.000 & 24.500 & 13.000 & \textbf{3.417}  & 19.667 & 38.250 & 3.083 & 2.750 & 1.250 & \textbf{0.000}  & 5.500 & 0.917 \\
$M_{\text{cs, loc}}(\rho = 0.1)$ & 0  & -  & -  & -  & -  & -  & -  & \textbf{0.000}  & 0.083 & \textbf{0.000}  & 0.083 & 0.167 & \textbf{0.000}  \\
$M_{\text{cs, loc}}(\rho = 0.1)$ & 3  & 1.417 & 8.750 & 2.250 & 2.833 & \textbf{1.167}  & 23.667 & \textbf{0.000}  & 0.167 & 0.083 & \textbf{0.000}  & 0.083 & 0.500 \\
$M_{\text{cs, loc}}(\rho = 0.4)$ & 0  & -  & -  & -  & -  & -  & -  & \textbf{0.000}  & \textbf{0.000}  & 0.250 & 0.167 & 0.583 & \textbf{0.000}  \\
$M_{\text{cs, loc}}(\rho = 0.4)$ & 3  & 1.250 & 9.750 & 10.417 & 11.667 & \textbf{0.250}  & 28.917 & \textbf{0.000}  & 0.167 & 0.167 & 0.167 & \textbf{0.000}  & 0.750 \\
$M_{\text{cs}}(\rho = 0.1)$ & 0  & -  & -  & -  & -  & -  & -  & 7.083 & 7.333 & 8.250 & \textbf{0.083}  & 24.500 & \textbf{0.083}  \\
$M_{\text{cs}}(\rho = 0.1)$ & 3  & 34.333 & 32.250 & 36.500 & \textbf{1.833}  & 18.333 & 25.083 & 5.167 & 5.167 & 6.250 & \textbf{0.000}  & 3.833 & 0.417 \\
$M_{\text{cs}}(\rho = 0.4)$ & 0  & -  & -  & -  & -  & -  & -  & 42.667 & 42.083 & 36.667 & 0.167 & 42.167 & \textbf{0.083}  \\
$M_{\text{cs}}(\rho = 0.4)$ & 3  & 46.750 & 46.583 & 46.333 & \textbf{18.250}  & 43.083 & 26.000 & 36.500 & 36.750 & 30.917 & \textbf{0.250}  & 33.167 & 0.667 \\
$M_{\text{AR}}(\rho = 0.1)$ & 0  & -  & -  & -  & -  & -  & -  & 54.500 & 41.333 & 61.000 & 0.500 & 23.083 & \textbf{0.167}  \\
$M_{\text{AR}}(\rho = 0.1)$ & 3  & 47.000 & 46.167 & 47.500 & \textbf{10.167}  & 44.917 & 43.917 & 51.500 & 37.167 & 56.500 & \textbf{0.167}  & 21.500 & 0.833 \\
$M_{\text{AR}}(\rho = 0.4)$ & 0  & -  & -  & -  & -  & -  & -  & 84.167 & 1.917 & 85.000 & 1.083 & 22.500 & \textbf{0.250}  \\
$M_{\text{AR}}(\rho = 0.4)$ & 3  & 47.833 & 43.000 & 47.917 & \textbf{17.833}  & 38.250 & 63.417 & 80.250 & 1.083 & 81.667 & \textbf{0.417}  & 19.417 & 1.500 \\
$M_{\text{async}}$ & 3  & 19.583 & 53.583 & 25.500 & 28.333 & \textbf{13.833}  & 38.250 & \textbf{0.250}  & 1.583 & 0.833 & 0.583 & 0.583 & 0.583 \\
$M_{\text{grad}}$ & 3  & 33.833 & 50.417 & 33.417 & 39.333 & \textbf{28.333}  & 41.000 & 1.000 & 1.750 & 0.917 & 0.833 & \textbf{0.500}  & 1.083 \\
\hline \\[-1.8ex]
\end{tabular}
\end{adjustbox}
\end{table}

